Detecting OODs as datapoints with High Uncertainty

Deep neural networks (DNNs) are known to produce incorrect predictions with very high confidence on out-of-distribution inputs (OODs). This limitation is one of the key challenges in the adoption of DNNs in high-assurance systems such as autonomous driving, air traffic management, and medical diagnosis. This challenge has received significant attention recently, and several techniques have been developed to detect inputs where the model's prediction cannot be trusted. These techniques detect OODs as datapoints with either high epistemic uncertainty or high aleatoric uncertainty. We demonstrate the difference in the detection ability of these techniques and propose an ensemble approach for detection of OODs as datapoints with high uncertainty (epistemic or aleatoric). We perform experiments on vision datasets with multiple DNN architectures, achieving state-of-the-art results in most cases.

==> MoE.tex <==
\section{Mixture of Experts for OOD Detection}
\label{sec:framework}
Equation~\ref{eq_ood_det} for the detection of OODs as data points with high uncertainty can be re-written as:
\begin{equation}
    \max (-\sum_{i=1}^{n_c} p_{i|x} \ \log\ p_{i|x} - \delta_a, \delta_{ep} - \max_{i=1}^{n_c}\{q_{pi}(x)\}) > 0
\end{equation}

A quantitative score to the OOD nature of an input $x$ can thus is assigned by:
\begin{equation}
    ood\_score(\delta_{a}, \delta_{ep}, \{p_{i|x}\}, \{q_{pi}\} | \ 1 \leq i \leq n_c ) = \max (-\sum_{i=1}^{n_c} p_{i|x} \ \log\ p_{i|x} - \delta_a, \delta_{ep} - \max_{i=1}^{n_c}\{q_{pi}(x)\})
\end{equation}

Logistic regression as gating network with two experts:\\
$P(expert = 1|x, v, v_0)=(1+\exp^{-(v^T x+v_{0})})^{-1}$

With $\eta=\{v_1,\ldots,v_m,v_{10},\ldots,v_{m0}\}$,

Softmax Gating network
$P(expert = j|x, \eta)=\frac{\exp(v^T_j x + v_{j0} )}{\sum_{j'=1}^{m}\exp(v^T_{j'} x + v_{j'0})}$

Gaussian Gating network
$P(expert = j|x, \eta)=\frac{\exp(-\frac{1}{2} (x-v_j)^T \sum_j^{-1} (x-v_j) )}{\sum_{j'=1}^{m}\exp(-\frac{1}{2} (x-v_{j'})^T \sum_{j'}^{-1} (x-v_{j'}) )}$

\begin{algorithm}[tb]
   \caption{MoE for detection of OODs as data points with high uncertainty}
   \label{algo:OODDetAlgo}
   \begin{algorithmic}
        \STATE {\bfseries Input:}{$ x, \{(\{p_{i|x}\}, \{q_{pi}\} | \ 1 \leq i \leq n_c )_{j}\ | \ 1 \leq j \leq m \}, \delta_a, \delta_{ep}, \delta, \eta$}
        \STATE {\bfseries Output:}{Is $x$ is an OOD?}
        \FOR{$j=1\ldots m$}
            \STATE $score_j = ood\_score(\delta_{a}, \delta_{ep}, (\{p_{i|x}\}, \{q_{pi}\} | \ 1 \leq i \leq n_c )_j)$
        
            \STATE  $isOOD = \sum_{j=1}^{n}P(expert=j|x,\eta) \times score_j$ 
        \ENDFOR
       \STATE return $isOOD > \delta$
    \end{algorithmic}
\end{algorithm}


% \begin{algorithm}
%     \SetAlgoLined
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{$ x, \{(\{p_{i|x}\}, \{q_{pi}\} | \ 1 \leq i \leq n_c )_{j}\ | \ 1 \leq j \leq m \}, \delta_a, \delta_{ep}, \delta, \eta$}
%     \Output{Is $x$ is an OOD?}
%     \For{$j=1\ldots m$}{
%      $score_j = ood\_score(\delta_{a}, \delta_{ep}, (\{p_{i|x}\}, \{q_{pi}\} | \ 1 \leq i \leq n_c )_j)$
%     }
%     $isOOD = \sum_{j=1}^{n}P(expert=j|x,\eta) \times score_j$ \\
%     return $isOOD > \delta$
%     \caption{MoE for detection of OODs as data points with high uncertainty}
%     \label{algo:OODDetAlgo}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noop{\begin{algorithm}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$ x, \delta, \delta_a, \delta_{ep}, \delta_{en}, M, \{q_{pi}\ | \ 1 \leq i \leq n_c \}, \{q_{ni}\ | \ 1 \leq i \leq n_c \},$}
    \Output{$ isOOD$}
     $\{p_{i|x} \ | \ 1 \leq i \leq n_c \} = M(x)$\\
     $au = -\sum_{i=1}^{n_c} p_{i|x} \ \log\ p_{i|x}$\\
     $\{eu_{pi}\} = \{q_{pi}(x) \ | \ 1 \leq i \leq n_c\}$\\
     $\{eu_{ni}\} = \{q_{ni}(x) \ | \ 1 \leq i \leq n_c \}$\\
     $isOOD = max (au - \delta_a,  \delta_{ep} - \max\{eu_{pi}\}, \delta_{en} - \max\{eu_{ni}(x)\}) > \delta$ \\
     return $isOOD$
    \caption{Detection of OODs due to aleatoric and epistemic uncertainty}
    \label{algo:OODDetAlgo}
\end{algorithm}


\begin{algorithm}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$x, \{p_i \ | \ 1 \leq i \leq n \}, \{ isOOD_i \ | \ 1 \leq i \leq n \}, f$}
    \Output{$isOOD$}
    %  $isOOD = \sum_i p_i \times isOOD_i$ \\
    $isOOD = f(\{p_i \ | \ 1 \leq i \leq n \}, \{isOOD_i \ | \ 1 \leq i \leq n \})$ \\
     return $isOOD$
 \caption{Mixture of Experts model for detection of OODs}
 \label{algo:moe}
\end{algorithm}
}


\noop{Mahalanobis distance of an input from the estimated ID density corresponds to measuring the log of the probability densities of the input~\citep{mahalanobis}. We, therefore use Mahalanobis distance from the tied ID to measure the epistemic uncertainty from Equation~\ref{eq_tied} in the first expert. PCA can be viewed as a maximum likelihood procedure on a Gaussian density model of the observed data~\citep{prob_pca}. We use the complementary property of PCA, which is minimizing error in the reconstruction of the input from the principal components (top 40\% eigen vectors), as the estimator of epistemic uncertainty in the second expert. We perform class-wise PCA analysis, i.e. using $max_{i=1}^{n_c}\{q_{pi}(x)\} < \delta_{ep} \vee False$ from Equation~\ref{eq_p_np_cc} to detect OODs due to high epistemic uncertainty in the second expert.

Logistic regression is one of the ways for determining and combining weights to the experts in the MoE~\citep{lr_moe}. We use logistic regression for determining $\{p_i \ | \ 1 \leq i \leq n \}$ and combining the determined weights in our experiments:
\begin{equation}
   f = \sum_i^{n}p_i \times isOODi
\end{equation}
}

\begin{comment}

The integrated OOD detection approach, thus, uses the following attributes, each specialized in detecting a specific type (or a combination of types) of OODs:

\begin{enumerate}[leftmargin=*]
    \item  Mahalanobis distance from the in-distribution density estimate that considers either tied~\citep{mahalanobis} or class-wise covariance estimate. This attribute captures  the overall or class-conditional epistemic uncertainty of an OOD. Our refinement to also use class-wise covariance significantly improves detection of OODs when coupled with PCA approach described below. 
    \item Conformance measure among the variance of the Annoy~\citep{annoy} nearest neighbors
    calculated as the Mahalanobis distance of the input's conformance to the closest class conformance. Our experiments found this to be very effective in capturing aleatoric uncertainty. This new attribute is a fusion of nearest-neighbor and Mahalanobis distance methods in literature.
    \item Prediction confidence of the classifier as the maximum softmax score on the perturbed input where the perturbation used is the same as ODIN approach~\citep{odin}. This boosts the detection of high aleatoric uncertainty by sharpening the class-wise distributions. 
    \item Reconstruction error using top  40\% of PCA components where the components are obtained via class conditional PCA of the training data. This boosts the detection of high class-wise epistemic uncertainty by eliminating irrelevant features. 
\end{enumerate}

This fusion of attributes from existing state-of-the-art detection methods and new attributes was found to be the most effective integrated appraoch capable of detecting the different types of OODs. We  evaluated it on several benchmarks as discussed in Section~\ref{sec:exp} with ablation study in Appendix.
\end{comment}

==> algo.tex <==
\begin{algorithm}[H]
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$x, \delta_a, \delta_e, q, M$}
    \Output{$isOOD$}
     $\{p_{1|x},\ldots,p_{n_c|x}\} = M(x)$\\
     $au = -\sum_{i=1}^{n_c} p_{i|x} \ log\ p_{i|x}$\\
     $eu = q(x)$\\
     $isOOD = au > \delta_a \vee eu < \delta_e$ \\
     return $isOOD$
 \caption{Detection of OODs due to uncertainty with tied ID}
\end{algorithm}


\begin{algorithm}[H]
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{$x, \delta_a, \delta_e, \{q_1,\ldots, q_{n_c}\}, M$}
    \Output{$isOOD$}
     $\{p_{1|x},\ldots,p_{n_c|x}\} = M(x)$\\
     $au = -\sum_{i=1}^{n_c} p_{i|x} \ log\ p_{i|x}$\\
     $\{eu_i\} = \{q_i(x)\} \ |\ 1\leq i \leq n_c$ \\
     $isOOD = au > \delta_a \vee max_{i=1}^{n_c} \{eu_i\} < \delta_e$ \\
     return $isOOD$
 \caption{Detection of OODs due to uncertainty with class-conditional ID}
\end{algorithm}


==> background.tex <==
\section{OOD detection from uncertainty point of view}
\label{sec:background}
Here we first define the two sources of uncertainty in 
the predictions of a classifier: epistemic and aleatoric uncertainty. We then discuss existing work on outlier detection based on these sources of uncertainty. \RK{Define OODs due to these two uncertainties (mainly aleatoric) and justify it - More related to low confident predictions for aleatoric uncertainty,  provenance, something related to abstaining on predictions?}

\textbf{Epistemic Uncertainty.} This form of uncertainty is caused due to the \textit{lack of knowledge}. Epistemic uncertainty in the predictions of a classifier is high in those regions where no data have been encountered so far. Low density regions of the training samples can thus be used as an indicator of high epistemic uncertainty~\citep{formal_eu_au, ML-uncertainty-survey}. This form of uncertainty can be reduced with more training data.

%For instance, uncertainty in the parameters of a classifier is due to the lack of knowledge about the perfect predictor, the Bayes-optimal classifier. Epistemic uncertainty can be reduced with more data used in training or learning the parameters of the classifier~\citep{ML-uncertainty-survey}. 

\textbf{Aleatoric Uncertainty.} This form of uncertainty is due to the \textit{inherent randomness} in the outcome, caused for instance by the noisy data. Since the dependency between the input set $\cal{X}$ and the output set $\cal{Y}$ is non-deterministic, the prediction $y \in \cal{Y}$ of a classifier on an input $x\in \cal{X}$ is a conditional probability distribution:
\begin{equation}
    p(y|x) = \frac{p(x,y)}{p(x)}
\end{equation}
This uncertainty in the prediction of a classifier is due to the aleatoric uncertainty. It can be reduced by adding more features (or attributes) to the data for distinguishing the classes~\citep{ML-uncertainty-survey}.

\textbf{Existing OOD detection methods based on uncertainty.} Using a threshold on the estimated density of the ID data has been used to detect OODs due to high epistemic uncertainty~\citep{mahalanobis, energy, ood_detect_density_eu}. In contrast, techniques based on the reasoning of the desired $p(y|x)$ for ID data focus on detection of OODs due to high aleatoric uncertainty~\citep{baseline,odin,kl-div}. 

==> classification_of_det_methods.tex <==
\section{Classification of OOD detection methods}
\label{sec:classification}
The low density regions in the modeled iD indicate high epistemic uncertainty~\citep{formal_eu_au,ML-uncertainty-survey}. The ability of the different techniques to detect different types of OODs can be explained by the focus of these techniques on measuring different sources of the epistemic uncertainty. We classify OOD detection techniques into two types based on their approach to capture different sources of epistemic uncertainty for OOD detection, namely discriminative and generative.

\textbf{Discriminative approach for OOD detection.}
Discriminative approach for OOD detection tries to capture high epistemic uncertainty due to those low density regions where entropy in the class prediction is high. Epistemic uncertainty is high in these ambiguous regions due to low evidence for the class prediction in these regions. This is caused by \textit{low sampling} of the true class from the iD in these regions. 
% Type 1 OODs in Figure~\ref{fig:OOD_types} are OODs due to high epistemic uncertainty in the low density regions where the entropy in the class label is high (class label can be 0 or 1).
\RK{Change lemmas to def/assumption - OODs due to one eu and OODs due to other eu...and then we compose them into a lemma}
\begin{lemma}
For a given threshold $\delta_d$ on the entropy in the predicted class distribution and $n_c$ as the number of classes, the discriminative approach detects an input $x$ as OOD if: 

\begin{equation}
    -\sum_{i=1}^{n_c} p_{i|x} \ \log\ p_{i|x} > \delta_d
\end{equation}
\end{lemma}

\textbf{Existing discriminative approaches for OOD detection. } SBP~\citep{baseline} uses maximum softmax probability as an indicator of the KL-divergence between distribution of the predicted softmax probabilities and the uniform distribution. This divergence measures entropy in the prediction of the class for an input~\citep{kl_div_entropy}. Therefore, SBP is able to detect those OODs which lie on or near the decision boundary (clusters $B$ and $C$) where it is least confident in its prediction. The predicted class distribution for an input can be obtained from any layer, and is not restricted to the softmax layer of the classifier. For instance,~\citet{dknn} use class labels of the nearest neighbors in the feature space (from all the layers) of the classifier for calculating entropy in the predicted class distribution for OOD detection. Therefore, this method is able to detect OODs with nearest neighbors from multiple classes (cluster $C$).
There are other techniques that are based on this discriminative approach for OOD detection~\citep{odin, kl-div, self-supervised, contrastive}.

\textbf{Generative approach for OOD detection.} Generative approach for OOD detection tries to capture high epistemic uncertainty due to those low density regions where \textit{no sampling} of the iD data points is done. These regions in the modeled iD can be due to two reasons. First, these regions are far from the true iD and therefore no samples are available for modeling the iD. Second, these regions are closer to the true iD but either no sampling is done or no samples are available in these regions.
This is different from the discriminative approach which tries to capture epistemic uncertainty in those regions where low sampling of the true class from the iD is done. 

% Generative approach makes use of the probability density function (PDF) $q$ representing the modeled iD density for OOD detection.

\begin{lemma}
For a given threshold $\delta_g$ on the probability of an input $x$ belonging to the modeled iD density $q$, the generative approach detects $x$ as OOD if:

\begin{equation}
    q(x) < \delta_g
\label{eq_tied}
\end{equation}
\label{lem:tied}
\end{lemma}

 

One can also consider either only principal (or non-principal) components in the PDF of the modeled iD to detect OODs due to high (or smaller) deviation in the principal (or non-principal) components of the modeled iD. 

\begin{lemma}
With $q_{p}$ (or $q_{n}$) as the PDF with only principal (or non-principal) components of the modeled iD and $\delta_{gp}$ (or $\delta_{gn}$) as the threshold on the probability of the input belonging to the modeled iD density due to the principal (or non-principal) components, generative approach detects an input $x$ as OOD if:
\begin{equation}
    q_{p}(x) < \delta_{gp} \vee q_{n}(x) < \delta_{gn}\  \textrm{where} \  \delta_{gp} > \delta_{gn}
\label{eq_p_np_tied}
\end{equation}
\label{lem:tied_p_np}
\end{lemma}

While considering only principal (or non-principal) components in the PDF of iD, the other term in the above equation corresponding to the non-principal (or principal) components is considered false. In other words, the input is assumed to be iD along those components for which it is not tested. However, if analysis is performed for both the components separately (instead of together as in Equation~\ref{eq_tied}), then the input is defined as an OOD if either of the two conditions in the above equation is true.

Note that $q(x)$ defined so far is for the tied (or single) iD. For class-conditional iD density, we will have a set $\{q_i(x)\ | \ 1 \leq i \leq n_c \}$ for PDFs for each class and thus the following lemmas. 

\begin{lemma}
Generative approach for OOD detection with class-conditional PDF set $\{q_i(x)\ | \ 1 \leq i \leq n_c \}$ detects an input $x$ as OOD if:

\begin{equation}
    \max_{i=1}^{n_c}\{q_i(x)\} < \delta_g
\label{eq_cc}
\end{equation}
\label{lem:cc}
\end{lemma}

\begin{lemma}
Generative approach considering only principal $\{q_{pi}(x)\ | \ 1 \leq i \leq n_c \}$ (or non-principal $\{q_{ni}(x)\ | \ 1 \leq i \leq n_c \}$) components in defining the modeled class-conditional iD density detects an input $x$ as OOD if:

\begin{equation}
    \max_{i=1}^{n_c}\{q_{pi}(x)\} < \delta_{gp} \vee \max_{i=1}^{n_c}\{q_{ni}(x)\} < \delta_{gn} \ \textrm{where} \  \delta_{gp} > \delta_{gn}
\label{eq_p_np_cc}
\end{equation}
\label{lem:cc_p_np}
\end{lemma}



Note that Equations~\ref{eq_tied} and~\ref{eq_p_np_tied} are the special case of Equations~\ref{eq_cc} and~\ref{eq_p_np_cc} respectively where the size of the sets representing the PDF of iD is equal to 1. Also, Equations~\ref{eq_tied} and~\ref{eq_cc} are a special case of Equations~\ref{eq_p_np_tied} and~\ref{eq_p_np_cc} respectively, when we do not consider dimensionality reduction, i.e. all components are considered as principal components in the PDF of iD. 

\textbf{Existing generative approaches for OOD detection. } Mahalanobis distance of an input from the estimated iD density corresponds to measuring the log of probability densities of an input~\citep{mahalanobis}. Using mahalanobis distance from the mean and covariance of all the training iD data detects OOD as a generative approach from Lemma~\ref{lem:tied}. This approach is therefore able to detect OODs lying in the low density region that is far from the tied iD (cluster A). PCA can be viewed as a maximum likelihood procedure on a Gaussian density model of the observed data~\citep{prob_pca}. Performing class-wise reconstruction error from PCA detects OODs as a generative approach from Lemma~\ref{lem:cc_p_np} with $\max_{i=1}^{n_c}\{q_{ni}(x)\} < \delta_{gn}$ equal to false as the analysis is performed along the principal components only. This approach is therefore able to detect OODs in the low density regions that are far from the modeled class-conditional iD (clusters A and B). There are other techniques that are based on this generative approach for OOD detection~\citep{oe,energy}. \RK{Does VAE/GAN based approach for OOD detection fall into this category? \\ https://link-springer-com.proxy.library.upenn.edu/content/pdf/10.1007/s10994-021-05946-3.pdf says that - density estimation is also a central building block in anomaly and outlier detection. Often, a threshold is applied on top of the density p(x) to decide
whether a data point is an outlier or not. For example, in auto-encoders, a low-dimensional
representation of the original input in constructed, and the reconstruction error can be used
as a measure of support of a data point within the underlying distribution.}



==> discussion.tex <==
\section{Discussion and future work}
\label{sec:dis}
Recent techniques propose refinement in the training process of the classifiers for OOD detection. Some of these techniques include fine-tuning the classifier's training with an auxiliary cost function for OOD detection~\citep{oe,energy}. Other techniques make use of self-supervised models for OOD detection~\citep{contrastive,self-supervised}. We perform preliminary experiments to compare the performance of these techniques with our integrated OOD detector that makes use of the feature space of the pre-trained classifiers to distinguish in-distribution samples from OODs. Our approach does not require modification of the training cost function of the original task. These results are reported in the Appendix. We consider making use of the feature space of in our OOD detection technique as a promising prospective future work. Another direction of the future work is to explore the score functions used in these refined training processes for OOD detection~\citep{energy,oe,contrastive,self-supervised} as attributes (or categories of attributes) forming the signature of the integrated OOD detector. Another avenue of future work is to explore OOD generation techniques other than adversarial examples generated by the FGSM attack for training of the integrated OOD detector. 





==> diversity.tex <==
\section{Diversity of OODs and Existing Detection Methods}
\label{sec:diversity}
\textbf{What are OODs/Empirical OOD?} Out-of-distribution data points are the points lying in the low density regions of the modeled in-distribution (iD). The modeled iD is learnt by training a classifier on the available iD dataset. So, OODs are defined with respect to the trained classifier and the observed (or sampled) data points from iD. \RK{Refer to papers for their usage of the term `OOD'. So use slightly different OOD because we do not have the true distribution? 2 aspects - uncertainty in true and modeled iD...clearly state what is done}

\textbf{Diversity of OODs.}  The low density regions can either be far or closer to the modeled iD~\citep{kl-div}. Low density regions that are far from the modeled iD are the regions with low (or no) iD data points despite high sampling from the iD. On the other hand, low density regions that are closer to the modeled iD are the regions with low iD data points that could be due to lower sampling of the iD data points in those regions. OODs can, thus, be of diverse types with respect to the type of the low density regions in which they lie.

OODs can be categorized as the data points lying far or closer to the modeled iD. OODs lying closer to the iD can further be categorized into OODs lying closer to one or multiple classes. 
Typical inputs to DNNs are high-dimensional and can be decomposed into principal and non-principal components based on the direction of high variation in the iD data. This yields another dimension for classification of OODs where the low density regions are defined either by unusually high deviation in the principal components or by smaller deviation in the non-principal (and hence, statistically invariant) components of the iD data. We can, thus, categorize an OOD using the following three criteria.

\begin{enumerate}
    \item Is the OOD a data point that is far or closer to the modeled iD?
    
    \item The OOD lying closer to the iD is close to one or multiple classes of the modeled iD?
    
    \item Is the OOD a data point due to high deviation in the principal or smaller deviation in the non-principal components of the modeled iD?
\end{enumerate}


\noop{\begin{figure}
   \begin{center}
    \includegraphics[width=0.5\textwidth]{figures/OOD_types.pdf}
    \caption{The different types of OODs in a 2D space with three iD classes. The class distributions are represented as Gaussians with black boundaries and the tied distribution of all training data is a Gaussian with red boundary.}
    \label{fig:OOD_types}
    \end{center}
\end{figure}

Figure~\ref{fig:OOD_types} demonstrates different types of OODs which differ along these criteria. Type 2 and 3 OODs are far from the modeled iD, whereas type 1, 4 and 5 OODs are closer to the modeled iD.  Type 1 OODs are closer to multiple classes (class 0 and class 1) whereas type 4 and 5 are close to single class (class 2 and class 1 respectively). Type 2 (or 4) and type 3 (or 5) differ from each other as they are OODs due to high variation in the principal and low variation in the non-principal components of the modeled iD data respectively.
\RK{Should we remove this figure?}}


\indent \textbf{Existing OOD Detection Methods.} 
Similar to the intuitions provided by~\citet{2d_intuition} on a two-dimensional (2D) toy problem to understand the behavior of uncertainty in high-dimensional image space, we also empirically demonstrate the limitations of existing OOD detection methods on a 2D half-moon dataset with two classes. 
%The samples from the two half-moons are in-distribution data. 
As shown in Figure~\ref{fig:toy_ex},
we consider three clusters of OOD samples: cluster A (black), B (brown) and C(red).
%(left). The trained DNN model comprises three fully connected layers. 
%\textcolor{red}{We consider a DNN classifier with three fully connected layers having 50, 2, and 2 neuron, respectively.} 
% Figure~\ref{fig:toy_ex} (right) shows the 2D penultimate features of the classifier. 

\begin{figure}[!h]
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.6\linewidth]{figures/taxonomy-sec/input_classifier_boundary.pdf}
  %\caption{} 
  %\label{fig:sfig1}
\end{subfigure}%
\quad
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.6\linewidth]{figures/taxonomy-sec/penul_input_with_OOD_types.pdf}
 % \caption{}
  %\label{fig:sfig1}
\end{subfigure}%
\caption{
%We use two half-moons to represent the distribution of the two classes in a 2D dataset. 
The cluster A (black), cluster B (brown), and  cluster C (red) clusters represent OODs that are \textit{far from iD, closer to one iD class and, closer to multiple iD classes} respectively.
(Left) shows the training data of the 2 half-moon classes and the 3 OOD clusters in the input space along with the trained classifier's boundary and its softmax scores. (Right) shows the ID samples and the OODs after projection to the 2D feature space (penultimate layer) of the DNN.} 
\label{fig:toy_ex}
\end{figure}


\begin{figure}[!h]
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Estimating distance from tied ID fails to detect OOD clusters B, C}
      {\includegraphics[width=.22\linewidth]{figures/taxonomy-sec/mahala_tied_dist_penul.pdf}}
%  \end{minipage}
  \quad
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Techniques based on softmax score fail to detect OOD cluster A}
      {\includegraphics[width=.22\linewidth]{figures/taxonomy-sec/base_classifier_boundary.pdf}}
%  \end{minipage}
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Estimating distance from class-wise ID fails to detect OODs cluster C}
      {\includegraphics[width=.22\linewidth]{figures/taxonomy-sec/pca_penul.pdf}}
%  \end{minipage}
  \quad
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Non-conformance in kNNs fails to detect OOD clusters A, B}
      {\includegraphics[width=.22\linewidth]{figures/taxonomy-sec/knn_label_conformance_penul.pdf}}
 % \end{minipage}
\caption{\textit{Different techniques fail to detect different types of OODs.}
}
\label{fig:failure_toy_ex}
\end{figure}

Different approaches differ in their ability to detect different OOD types, as illustrated in Figure~\ref{fig:failure_toy_ex}.
\begin{itemize}[topsep=0pt,leftmargin=*]

    \item Figure~\ref{fig:failure_toy_ex}(a) shows that the  Mahalanobis distance~\citep{mahalanobis} from the mean and covariance of all the training data in the feature space cannot detect OODs lying closer to the modeled iD. It attains the overall true negative rate (TNR) of 39.09\% at  the 95\% true positive rate (TPR). 
    
     \item Figure~\ref{fig:failure_toy_ex}(b) shows that the softmax prediction probability (SPB)~\citep{baseline} cannot  detect the OODs lying far from the modeled iD. The TNR ( at 95\% TPR) reported by the SPB technique is 60.91\%.  
     \item Figure~\ref{fig:failure_toy_ex}(c) shows that class-wise Principal Component Analysis (PCA)~\citep{pca} cannot detect OODs closer to multiple classes. We performed PCA of the two classes separately in the  feature space and used the minimum reconstruction error to detect OODs. 
     This obtained overall TNR of 80.91\% (at 95\% TPR). 
     \item Figure~\ref{fig:failure_toy_ex}(d) shows that non-conformance in the labels of the K-Nearest Neighbors (kNNs)~\citep{dknn} 
     \RK{(the value of k=10)} cannot detect OODs lying far and closer to one class of the modeled iD. The overall TNR (at 95\% TPR) reported by this technique is 15\%. 
\end{itemize} 


==> framework.tex <==
\section{Integrated OOD Detection Method}
\label{sec:framework}
Complementary information about different OOD types can be used to detect a wider range of OODs. Figure~\ref{fig:framework_toy_ex} shows the improvement in the TNR of the OOD detector composed with information about different classes of OODs on the two half-moons dataset. Non-conformity in the labels of the nearest neighbors captures OODs in cluster C. Mahalanobis distance from the tied in-distribution detects OODs in cluster A. Reconstruction error from the PCA of the 2 class distributions captures OODs in cluster B. Softmax scores further strengthens the OOD detection by reporting OODs in cluster C that are undetected by the other three methods.

\begin{figure}[!h]
%  \centering
%  \begin{minipage}{.48\linewidth}
    \centering
   % \subcaptionbox{\textbf{15\% TNR} with non-conformance among the labels of the nearest neighbors}
      {\includegraphics[width=.35\linewidth]{figures/integrated-sec/knn_label_conf_input.pdf}}
%  \end{minipage}\quad
%  \begin{minipage}{.48\linewidth}
    \centering
%    \subcaptionbox{\textbf{54.09\% TNR} with non-conformance measure among the labels of the nearest neighbors and mahalanobis distance from the tied in-distribution to detect OODs}
      {\includegraphics[width=.35\linewidth]{figures/integrated-sec/knn_label_conf+mahala_tied_dist_input.pdf}}
%  \end{minipage}
%  \begin{minipage}{.48\linewidth}
    \centering
%    \subcaptionbox{\textbf{95.91\% TNR} with non-conformance measure among the labels of the nearest neighbors, mahalanobis distance from the tied in-distribution and reconstruction error from PCA of the two classes to detect OODs}
      {\includegraphics[width=.35\linewidth]{figures/integrated-sec/knn_label_conf+mahala_tied_dist+pca_input.pdf}}
 % \end{minipage}\quad
 % \begin{minipage}{.48\linewidth}
    \centering
 %   \subcaptionbox{\textbf{99.55\% TNR}  with non-conformance measure among the labels of the nearest neighbors, mahalanobis distance from the tied in-distribution, reconstruction error from PCA of the two classes and the classifier's softmax scores to detect OODs}
      {\includegraphics[width=.35\linewidth]{figures/integrated-sec/knn_label_conf+mahala_tied_dist+pca+baseline_input.pdf}}
 % \end{minipage}
\caption{Complementary information about different types of OODs improves detection. (Top-left) \textbf{15\%} TNR with non-conformance among the labels of the nearest neighbors. (Top-right) Adding Mahalanobis distance over the tied in-distribution improves TNR to \textbf{54.09\%}. (Bottom-left) Adding Class-wise PCA further improves TNR to  \textbf{95.91\%} TNR. (Bottom-right) Adding softmax score further improves TNR to \textbf{99.55\%}. TPR is 95\% in all the cases.}
\label{fig:framework_toy_ex}
\end{figure}

\noop{
If $\newinp$ is an OOD, we can identify it answering the following three questions: 

\begin{enumerate}[noitemsep,topsep=0pt,leftmargin=*]
    \item Is the OOD input having higher epistemic or aleatoric uncertainty, that is, is the input away from all training data or is it unusually more confusing? 
    \\ \RK{The answer for the epistemic is given by the Mahalanobis distance (with class-wise mean and tied or class-wise variance). The answer for the aleatoric is given by the NN conformance and the softmax score. Do we need to answer why are we using 2 features for answering aleatoric uncertainty question? If so, then we can say that as observed from the experiment on toy dataset, softmax adds complementary strength to the NN method by detecting those OODs which NN missed.}
    \item Is the epistemic uncertainty of the OOD input unconditional or it it conditioned on the class predicted by the DNN model?
    \item Is the OOD an outlier due to unusually high deviation in the principal components of the data or due to small deviation in the non-principal (and hence, invariant) components? 
    \\ \RK{The answer for 2 and 3 are given by the reconstruction error of the PCA in the class-conditional distribution of the training data.}
\end{enumerate}
}

The integrated OOD detection approach, thus, uses the following attributes, each specialized in detecting a specific type (or a combination of types) of OODs:

\begin{enumerate}[leftmargin=*]
    \item  Mahalanobis distance from the in-distribution density estimate that considers either tied~\citep{mahalanobis} or class-wise covariance estimate. This attribute captures  the overall or class-conditional epistemic uncertainty of an OOD. Our refinement to also use class-wise covariance significantly improves detection of OODs when coupled with PCA approach described below. 
    \item Conformance measure among the variance of the Annoy~\citep{annoy} nearest neighbors
    calculated as the Mahalanobis distance of the input's conformance to the closest class conformance. Our experiments found this to be very effective in capturing aleatoric uncertainty. This new attribute is a fusion of nearest-neighbor and Mahalanobis distance methods in literature.
    \item Prediction confidence of the classifier as the maximum softmax score on the perturbed input where the perturbation used is the same as ODIN approach~\citep{odin}. This boosts the detection of high aleatoric uncertainty by sharpening the class-wise distributions. 
    \item Reconstruction error using top  40\% of PCA components where the components are obtained via class conditional PCA of the training data. This boosts the detection of high class-wise epistemic uncertainty by eliminating irrelevant features. 
\end{enumerate}

This fusion of attributes from existing state-of-the-art detection methods and new attributes was found to be the most effective integrated appraoch capable of detecting the different types of OODs. We  evaluated it on several benchmarks as discussed in Section~\ref{sec:exp} with ablation study in Appendix.

\noop{
While mahalanobis distance estimation with tied covariance and SPB attributes are used by the existing state-of-the-art OOD detection methods, we introduce two new attributes based on the mahalanobis distance estimate with class covariance and conformance measure among the variance of nearest neighbors to enhance the detection on all identified types of OODs by capturing both epistemic and aleatoric uncertainty.

These attributes are selected such that the framework satisfies the following two properties: 
\begin{enumerate}
    \item \textbf{Sound:} This property is with respect to the choice of attributes in the framework. Each attribute should be able to differentiate in-distribution samples from at least one class of OODs from its taxonomy.
    \begin{equation}
        \forall \text{attribute} \in \text{framework}, \exists \text{OOD type} \in \text{taxonomy},
        \text{s.t. attribute captures differentiating property of the OOD type}...
    \end{equation}
    \item \textbf{Complete:} This property is with respect to the three classes of OODs defined in its taxonomy. Each class of OOD should have at least one attribute in the framework that tries to differentiate in-distribution samples from OODs belonging to that class.
    \begin{equation}
            \forall \text{OOD type} \in \text{taxonomy}, \exists \text{attribute} \in \text{framework}, \text{s.t. the property differentiating the OOD type is captured by the attribute}
    \end{equation}
\end{enumerate}

% Based on this observation, we divide our features into four groups: features capturing the signature of OODs due to aleatory uncertainty (AU), features capturing the signature of epistemic uncertainty in tied in-distribution (EUT), features capturing the signature of epistemic uncertainty in class-wise in-distribution (EUC) and others (O). An OOD detector will be trained on all four feature subsets. Thus a feature vector x is made up of four parts: $x = [x_{AU},\ x_{EUT},\ x_{EUC},\ x_{O}]$. We use $f(x)$ to denote the output of the detector.

The weighted sum of these $n$ attributes in the framework forms a signature differentiating in-distribution samples from a diverse set of OODs:

\begin{equation}
    Signature(OOD\ detector) = \sum_{i=1}^n w_i \times \text{attribute}_{i}
\end{equation}

As illustrated in the experimental section, an OOD detector based on this signature out-performs the state of the art OOD detectors by capturing a wider range of OODs on several benchmarks.

}

==> integrated_approach.tex <==
\section{Mixture of Experts Model to Detect OODs}
\label{sec:framework}
Complementary information about different OOD types can be used to detect a wider range of OODs. Figure~\ref{fig:framework_toy_ex} shows the improvement in the TNR of the OOD detector composed with information about different classes of OODs on the two half-moons dataset. Non-conformity in the labels of the nearest neighbors captures OODs in cluster C. Mahalanobis distance from the tied in-distribution detects OODs in cluster A. Reconstruction error from the PCA of the 2 class distributions captures OODs in cluster B. Softmax scores further strengthens the OOD detection by reporting OODs in cluster C that are undetected by the other three methods.

\begin{figure}[!h]
%  \centering
%  \begin{minipage}{.48\linewidth}
    \centering
   % \subcaptionbox{\textbf{15\% TNR} with non-conformance among the labels of the nearest neighbors}
      {\includegraphics[width=.35\linewidth]{figures/integrated-sec/knn_label_conf_input.pdf}}
%  \end{minipage}\quad
%  \begin{minipage}{.48\linewidth}
    \centering
%    \subcaptionbox{\textbf{54.09\% TNR} with non-conformance measure among the labels of the nearest neighbors and mahalanobis distance from the tied in-distribution to detect OODs}
      {\includegraphics[width=.35\linewidth]{figures/integrated-sec/knn_label_conf+mahala_tied_dist_input.pdf}}
%  \end{minipage}
%  \begin{minipage}{.48\linewidth}
    \centering
%    \subcaptionbox{\textbf{95.91\% TNR} with non-conformance measure among the labels of the nearest neighbors, mahalanobis distance from the tied in-distribution and reconstruction error from PCA of the two classes to detect OODs}
      {\includegraphics[width=.35\linewidth]{figures/integrated-sec/knn_label_conf+mahala_tied_dist+pca_input.pdf}}
 % \end{minipage}\quad
 % \begin{minipage}{.48\linewidth}
    \centering
 %   \subcaptionbox{\textbf{99.55\% TNR}  with non-conformance measure among the labels of the nearest neighbors, mahalanobis distance from the tied in-distribution, reconstruction error from PCA of the two classes and the classifier's softmax scores to detect OODs}
      {\includegraphics[width=.35\linewidth]{figures/integrated-sec/knn_label_conf+mahala_tied_dist+pca+baseline_input.pdf}}
 % \end{minipage}
\caption{Complementary information about different types of OODs improves detection. (Top-left) \textbf{15\%} TNR with non-conformance among the labels of the nearest neighbors. (Top-right) Adding Mahalanobis distance over the tied in-distribution improves TNR to \textbf{54.09\%}. (Bottom-left) Adding Class-wise PCA further improves TNR to  \textbf{95.91\%} TNR. (Bottom-right) Adding softmax score further improves TNR to \textbf{99.55\%}. TPR is 95\% in all the cases.}
\label{fig:framework_toy_ex}
\end{figure}

\noop{
If $\newinp$ is an OOD, we can identify it answering the following three questions: 

\begin{enumerate}[noitemsep,topsep=0pt,leftmargin=*]
    \item Is the OOD input having higher epistemic or aleatoric uncertainty, that is, is the input away from all training data or is it unusually more confusing? 
    \\ \RK{The answer for the epistemic is given by the Mahalanobis distance (with class-wise mean and tied or class-wise variance). The answer for the aleatoric is given by the NN conformance and the softmax score. Do we need to answer why are we using 2 features for answering aleatoric uncertainty question? If so, then we can say that as observed from the experiment on toy dataset, softmax adds complementary strength to the NN method by detecting those OODs which NN missed.}
    \item Is the epistemic uncertainty of the OOD input unconditional or it it conditioned on the class predicted by the DNN model?
    \item Is the OOD an outlier due to unusually high deviation in the principal components of the data or due to small deviation in the non-principal (and hence, invariant) components? 
    \\ \RK{The answer for 2 and 3 are given by the reconstruction error of the PCA in the class-conditional distribution of the training data.}
\end{enumerate}
}

The integrated OOD detection approach, thus, uses the following attributes, each specialized in detecting a specific type (or a combination of types) of OODs:

\begin{enumerate}[leftmargin=*]
    \item  Mahalanobis distance from the in-distribution density estimate that considers either tied~\citep{mahalanobis} or class-wise covariance estimate. This attribute captures  the overall or class-conditional epistemic uncertainty of an OOD. Our refinement to also use class-wise covariance significantly improves detection of OODs when coupled with PCA approach described below. 
    \item Conformance measure among the variance of the Annoy~\citep{annoy} nearest neighbors
    calculated as the Mahalanobis distance of the input's conformance to the closest class conformance. Our experiments found this to be very effective in capturing aleatoric uncertainty. This new attribute is a fusion of nearest-neighbor and Mahalanobis distance methods in literature.
    \item Prediction confidence of the classifier as the maximum softmax score on the perturbed input where the perturbation used is the same as ODIN approach~\citep{odin}. This boosts the detection of high aleatoric uncertainty by sharpening the class-wise distributions. 
    \item Reconstruction error using top  40\% of PCA components where the components are obtained via class conditional PCA of the training data. This boosts the detection of high class-wise epistemic uncertainty by eliminating irrelevant features. 
\end{enumerate}

This fusion of attributes from existing state-of-the-art detection methods and new attributes was found to be the most effective integrated appraoch capable of detecting the different types of OODs. We  evaluated it on several benchmarks as discussed in Section~\ref{sec:exp} with ablation study in Appendix.

\noop{
While mahalanobis distance estimation with tied covariance and SPB attributes are used by the existing state-of-the-art OOD detection methods, we introduce two new attributes based on the mahalanobis distance estimate with class covariance and conformance measure among the variance of nearest neighbors to enhance the detection on all identified types of OODs by capturing both epistemic and aleatoric uncertainty.

These attributes are selected such that the framework satisfies the following two properties: 
\begin{enumerate}
    \item \textbf{Sound:} This property is with respect to the choice of attributes in the framework. Each attribute should be able to differentiate in-distribution samples from at least one class of OODs from its taxonomy.
    \begin{equation}
        \forall \text{attribute} \in \text{framework}, \exists \text{OOD type} \in \text{taxonomy},
        \text{s.t. attribute captures differentiating property of the OOD type}...
    \end{equation}
    \item \textbf{Complete:} This property is with respect to the three classes of OODs defined in its taxonomy. Each class of OOD should have at least one attribute in the framework that tries to differentiate in-distribution samples from OODs belonging to that class.
    \begin{equation}
            \forall \text{OOD type} \in \text{taxonomy}, \exists \text{attribute} \in \text{framework}, \text{s.t. the property differentiating the OOD type is captured by the attribute}
    \end{equation}
\end{enumerate}

% Based on this observation, we divide our features into four groups: features capturing the signature of OODs due to aleatory uncertainty (AU), features capturing the signature of epistemic uncertainty in tied in-distribution (EUT), features capturing the signature of epistemic uncertainty in class-wise in-distribution (EUC) and others (O). An OOD detector will be trained on all four feature subsets. Thus a feature vector x is made up of four parts: $x = [x_{AU},\ x_{EUT},\ x_{EUC},\ x_{O}]$. We use $f(x)$ to denote the output of the detector.

The weighted sum of these $n$ attributes in the framework forms a signature differentiating in-distribution samples from a diverse set of OODs:

\begin{equation}
    Signature(OOD\ detector) = \sum_{i=1}^n w_i \times \text{attribute}_{i}
\end{equation}

As illustrated in the experimental section, an OOD detector based on this signature out-performs the state of the art OOD detectors by capturing a wider range of OODs on several benchmarks.

}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> rel.tex <==
\section{Related work}
\label{sec:rel}
\begin{itemize}
    \item Existing work - On single distinguishing feature of OODs from IDs from intro

    Recent approaches for OOD detection consider different statistical, geometric or topological  signatures in data that  
    differentiate OODs from the training distribution. For example, the changes in the softmax scores due to input perturbations and temperature scaling have been used to detect OODs~\citep{baseline, odin, temp-scaling}. \citet{dknn} use the conformance among the labels of the nearest neighbors while \citet{contrastive} use cosine similarity (modulated by the norm of the feature vector) to the nearest training sample for the detection of OODs. \citet{mahalanobis} consider the Mahalanobis distance of an input from the in-distribution data to detect OODs. Several other metrics such as reconstruction error~\citep{vae-recon-err}, likelihood-ratio between the in-distribution and OOD samples~\citep{likelihood-ratio}, trust scores (ratio of the distance to the nearest class different from the predicted class and the distance to the predicted class)~\citep{trust-score}, density function~\citep{energy, oe}, probability distribution of the softmax scores~\citep{kl-div,self-supervised,contrastive} have also been used to detect OODs. All these methods attempt to develop a uniform approach with a single signature to detect all OODs accompanied by empirical evaluations that use datasets such as CIFAR10 as in-distribution data and other datasets such as SVHN as OOD. 
    \item Check if anyone else has tried to classify OOD detection techniques as generative VS discriminative
    \item Compare with the most recent work from discussion section and the other paper
    \item \href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9144212&tag=1}{} It has tried to list down the strengths and weakness of OOD and adversarial detectors, there is another paper that uses two types of distinguishing features for detection of adversarial examples-  logistic regression classifier with two features as input: the uncertainty and the density estimate- https://arxiv.org/pdf/1703.00410.pdf 
\end{itemize}

==> taxonomy-old.tex <==

\section{OOD Taxonomy and Existing Detection Methods}
\label{sec:taxonomy}
We consider a DNN, trained on the in-distribution samples, to detect OOD samples. Based on the uncertainties associated with the samples, we characterize ODD samples in two categories: epistemic and aleatoric~\citep{uncertainty, ML-uncertainty-survey}. 

\noop{
Beyond the simple characterization of OOD samples as anomalous inputs with respect to the training data, we 
%adopt the top-down inference for a more fine-grained definition of OOD that 
take into account the prediction of the DNN model on the input in determining whether it is OOD or not. This ensures 
%we can take into account 
characterizing both the epistemic and aleatoric uncertainty~\citep{uncertainty}.
%and enables the use of distributions learned individually over the training samples of each class along with the tied distribution learned across classes.
}



\begin{wrapfigure}{r}{0.6\textwidth}
%  \begin{minipage}[c]{0.7\textwidth}
   \begin{center}
    \includegraphics[width=0.6\textwidth]{figures/ood_types_dist_boundary.pdf}
    \caption{The different types of OODs in a 2D space with three different classes. The class distributions are represented as Gaussians with black boundaries and the tyied distribution is a Gaussian with red boundary. }
    \label{fig:OOD_types}
       \end{center}
%  \end{minipage}
 %\begin{minipage}[c]{0.5\textwidth}
%\end{minipage}
%\end{figure}
\end{wrapfigure}

\AR{
\indent \textbf{Taxonomy of OODs.}
%Uncertainty in the prediction of a classifier can be used to detect OODs. We consider aleatory and epistemic as the two sources of this uncertaint. 
% Epistemic uncertainty arises due to the lack of the classifier's knowledge (such as limited training data) whereas aleatory uncertainty is due to the stochasticity (or randomness) involved in its prediction.  
Given a test sample, we analyze the DNN's prediction compared to the in-distribution class boundaries. An OOD sample is associated with aleatoric uncertainty when the DNN may confuse the sample with multiple in-distribution classes (Type 3 OODs in Fig.~\ref{fig:OOD_types}). In case of the epistemic uncertainty, a sample is less likely to belong any of the in-distribution classes (Type 1 OODs in Fig.~\ref{fig:OOD_types}). The uncertainty in the classifier's prediction can thus be quantified with a distance measure from the distribution(s) of the in-distribution samples. \RK{Do we want t osay something about OOD Type 2 here?}

In case of epistemic uncertainty, either a single distribution is estimated for all the in-distribution samples or a class-wise distribution is estimated to capture conditional epistemic uncertainty. Based on the conditional epistemic uncertainty, epistemic uncertainty can be further divided into two types: \textcolor{red}{1) with high variance along the principal components, 2) with relatively low variance across invariant components.}

To this end, we identify an OOD using the following three criteria. 
\begin{enumerate}[noitemsep,topsep=0pt,leftmargin=*]
    \item Is the OOD samples are associated with higher epistemic or aleatoric uncertainty, i.e., is the input away from all in-distribution data or can it be confused between multiple classes? 
    \item Is the epistemic uncertainty of an OOD sample is unconditional or it it conditioned on the class predicted by the DNN model?
    \item Is the OOD an outlier due to unusually high deviation in the principal components of the data or due to small deviation in the non-principal (and hence, invariant) components? 
\end{enumerate}

Figure~\ref{fig:OOD_types} demonstrates different types of OOD which differ along these criteria. Type 1 OOD samples have high epistemic uncertainty and are away from the in-distribution data. Type 2 OOD samples have high epistemic uncertainty with respect to each of the 3 classes even though approximating distribution of all in-distribution data will miss these outliers. Type 3 OOD samples have high aleatoric uncertainty as they are close to the decision boundary between class 0 and class 1. Type 4 and 5 have high epistemic uncertainty with respect to the closest class. While Type 4 OOD samples are far from the distribution along the principal axis, Type 5  OOD samples vary along a relatively invariant axis where even a small deviation indicates an OOD. 

In general, for $k$ number of classes $c_1, c_2, \ldots, c_k$, we denote the distribution of training data for each class as $p(x | c_i)$. The overall training distribution is denoted by $p(x)$. Given a new input $\newinp$ to the trained DNN model $M$, let $\newclass = M(\newinp)$ denote the predicted class. The flowchart in Figure~\ref{fig:OOD_flow} shows the steps to determine whether $\newinp$ is an OOD sample.
}




\noop{
\indent \textbf{Taxonomy of OODs. }
%Uncertainty in the prediction of a classifier can be used to detect OODs. We consider aleatory and epistemic as the two sources of this uncertaint. 
% Epistemic uncertainty arises due to the lack of the classifier's knowledge (such as limited training data) whereas aleatory uncertainty is due to the stochasticity (or randomness) involved in its prediction.  
DNN models predict the class of a new input based on the learned classification boundaries between the distribution of the training samples of different classes. Aleatory uncertainty occurs in the regions where these distributions overlap for multiple classes, and epistemic uncertainty occurs in the regions where the probability of a sample belonging to any of the class distributions is low~\citep{ML-uncertainty-survey}. 
The uncertainty in the classifier's prediction can thus be quantified with a distance measure from the distribution(s) of the training samples. A sample lying close to multiple classes forms the source of aleatory uncertainty and a sample lying far from all the class distributions forms the source of epistemic uncertainty. In the latter case, the distribution of the training samples can be approximated either by a single tied distribution of the entire dataset or class-wise distributions defined by different classes in the dataset. The OODs due to high conditional epistemic uncertainty can be further divided into two types - those with high variance along the principal components and those with relatively low variance across invariant components.
We can thus identify an OOD using the following three criteria. 
\begin{enumerate}[noitemsep,topsep=0pt,leftmargin=*]
    \item Is the OOD input having higher epistemic or aleatoric uncertainty, that is, is the input away from all training data or is it unusually more confusing? 
    \item Is the epistemic uncertainty of the OOD input unconditional or it it conditioned on the class predicted by the DNN model?
    \item Is the OOD an outlier due to unusually high deviation in the principal components of the data or due to small deviation in the non-principal (and hence, invariant) components? 
\end{enumerate}

Figure~\ref{fig:OOD_types} demonstrates different types of OOD which differ along these criteria. Type 1 OODs have high epistemic uncertainty and are away from the training data. Type 2 OODs have high epistemic uncertainty with respect to each of the 3 classes even though approximating distribution of all training data will miss these outliers. Type 3 OODs have high aleatoric uncertainty as they are close to the decision boundary between class 0 and class 1. Type 4 and 5 have high epistemic uncertainty with respect to the closest class. While Type 4 OODs are far from the distribution along the principal axis, Type 5  OODs vary along a relatively invariant axis where even a small deviation indicates an OOD. 

\noop{
In general, 
let there be $k$ classes $c_1, c_2, \ldots, c_k$ and the distribution of training data for each class is $p(x | c_i)$. The overall training distribution is denoted by $p(x)$. Now, given a new input $\newinp$ to the trained DNN model $M$, let $\newclass = M(\newinp)$ denote the predicted class. The flowchart in Figure~\ref{fig:OOD_flow} shows different sources of uncertainty that could make  $\newinp$ an OOD.
}


\begin{figure}[!h]
\centering
\includegraphics[scale=.45]{figures/OOD-flow.png}
\caption{OODs with High Epistemic and Aleatoric Uncertainty} 
\label{fig:OOD_flow}
\end{figure}
}



\noop{
Table~\ref{table:OOD_types} summarizes the taxonomy of OODs based on the distance from the in-distribution and the source of uncertainty. In case of a single tied in-distribution, the only source of uncertainty is the epistemic uncertainty. We classify those samples that lie far from the approximated tied in-distribution as the OODs due to the epistemic uncertainty in the tied in-distribution. Examples of these types of OODs are shown as the black colored OODs in Figure~\ref{fig:OOD_types}. In case of class-wise distribution of the training samples, both epistemic and aleatory can be the source of uncertainty. We classify the samples lying close to multiple class distributions as the OODs due to the aleatory uncertainty in the class-wise in-distribution. Examples of these OODs are shown as the red colored OODs in Figure~\ref{fig:OOD_types}. Those samples that lie far from all the class distributions are classified as the OODs due to the epistemic uncertainty in the class-wise distribution of the in-distribution. 
\begin{table}[!h]
\caption{Taxonomy of OODs}
\label{sample-table}
\begin{center}
\begin{tabular}{lll}
\multicolumn{1}{c}{\bf OOD Type}  &\multicolumn{1}{c}{\bf Source of uncertainty}
\\ \hline \\
Far from tied in-distribution                                   & Epistemic\\
Far from all classes in class-wise in-distribution              & Epistemic\\
Close to multiple class in class-wise in-distribution           & Aleatory\\

\end{tabular}
\end{center}
\label{table:OOD_types}
\end{table}
}


%##########################################################################
%##########################################################################
%##########################################################################


%\subsection{Decomposed Distribution of OODs}

%Further, the OOD due to high epistemic uncertainty can be further divided into two types - those detected by tied distribution across classes and those that are far from all individual classes but not detected by tied distribution due to approximation. The OODs due to high conditional epistemic uncertainty can be further divided into two types - those with high variance along the principal components and those with relatively low variance across invariant components. %These 5 types of OODs are shown in Figure~\ref{fig:OOD_types}. 

%While measuring the distance of a new sample from the learned distribution to estimate $p(\newinp|\newclass)$, we can decompose the input and the training data into a set of orthogonal components and then weigh the component-wise distance from the learned distributions based on the variance of training data along different components. Outliers can have small variance around invariant components or unusually large variance around principle components.
%Decomposing the data along different components with different levels of variation in the training data enables decomposed specification of outliers, and 
%Directly computing outlier metrics such as Mahalanobis distance in the original dimensions of the input does not distinguish between .





%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################


%Three blobs of data-points representing the three types of OODs were used in this example. 

\indent \textbf{Prior Work: Limitations of \textbf{UNIFORM} Detection Methods.} We empirically demonstrate the limitations of existing \RK{not sure if we should say existing or uniform OOD detection techniques} OOD detection methods on a two-dimensional (2D) half-moon dataset with two classes. We assume the samples from the two half-moons to be ID and consider three clusters of OOD samples as shown in Fig.~\ref{fig:toy_ex} (left). \textcolor{red}{We consider a DNN classifier with three fully connected layers having 50, 2, and 2 neuron, respectively.} Figure~\ref{fig:toy_ex} (right) shows the 2D penultimate features of the classifier. The cluster A (black), cluster B (brown), and  cluster C (red) clusters represent the OOD due to epistemic uncertainty in the \textcolor{red}{tied ID}, epistemic uncertainty in the class-conditional ID and aleatoric uncertainty in the class-conditional ID, respectively.

\begin{figure}[!h]
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{figures/taxonomy-sec/input_classifier_boundary.pdf}
  %\caption{} 
  %\label{fig:sfig1}
\end{subfigure}%
\quad
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{figures/taxonomy-sec/penul_input_with_OOD_types.pdf}
 % \caption{}
  %\label{fig:sfig1}
\end{subfigure}%
\caption{We use two half-moons to represent the distribution of the two classes in a 2D dataset. (Left) shows the ID samples and the three clusters of OODs in the input space with the trained classifier's boundary and its softmax scores. (Right) shows the ID samples and the OODs in the 2D penultimate feature space of the classier.} 
\label{fig:toy_ex}
\end{figure}


\begin{figure}[!h]
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the density estimation technique of tied in-distribution to detect OODs in cluster B and C.}
      {\includegraphics[width=.4\linewidth]{figures/taxonomy-sec/mahala_tied_dist_penul.pdf}}
%  \end{minipage}
  \quad
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the softmax score based technique to detect OODs in cluster A}
      {\includegraphics[width=.4\linewidth]{figures/taxonomy-sec/base_classifier_boundary.pdf}}
%  \end{minipage}
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the density estimation technique of the class-wise in-distribution to detect OODs in cluster C}
      {\includegraphics[width=.4\linewidth]{figures/taxonomy-sec/pca_penul.pdf}}
%  \end{minipage}
  \quad
%  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the non-conformance among the nearest neighbors to detect OODs in cluster A and B}
      {\includegraphics[width=.4\linewidth]{figures/taxonomy-sec/knn_label_conformance_penul.pdf}}
 % \end{minipage}
\caption{Different detection techniques differ in their ability to detect different types of OODs. We call OODs due to epistemic uncertainty in tied ID, class-conditional epistemic uncertainty and aleatoric uncertainty as OODs in cluster A, B and C respectively.}
\label{fig:failure_toy_ex}
\end{figure}



Different approaches differ in their ability to detect different classes of OODs. % described in the previous section. 
First, detection techniques based on density estimation of the tied ID of all the training data do not consider the class of datapoints. Hence, these cannot detect OODs due to the aleatory or epistemic uncertainty in the class-wise distribution.
The estimated tied distribution is overapproximate and it also cannot recognize confusing inputs between different classes.
%over-approximates the in-distribution data  to learn a single distribution and cannot recognize inputs as being confusing between different classes. 
Second, OOD detection techniques based on the softmax prediction probability(SPB) can detect OODs with high aleatoric uncertainty and inter-class confusion. But these are unable to detect the OODs with epistemic uncertainty in the tied ID. This is because of the high softmax scores usually assigned to the samples lying far from the classification boundary by the DNN classifiers. 
Third, OOD detection techniques based on density estimation of the class-wise ID might not be able to detect OODs with high aleatory uncertainty unless we perform counterfactual analysis with classes alternative to the predicted class. 
%OOD detection techniques for class-wise in-distribution 
Finally, the techniques based on the non-conformance amongst the properties of the nearest neighbors from the training samples might not be able to detect OODs due to epistemic uncertainty (in class-wise or tied in-distribution) whose nearest neighbors belong to the same class. 
%This is because training samples from the same class are expected to be conformant in their properties. 

Using the toyset, we empirically demonstrated these limitations of existing OOD detection techniques as summarized in Figure~\ref{fig:failure_toy_ex}. 
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=*]
    \item Mahalanobis distance~\citep{mahalanobis}: 
     A variation in the Mahalanobis distance based method is considered here. Instead of using class-conditional mean and tied covariance, tied mean and tied covariance of all the training data in the penultimate feature space is considered here. This is done to estimate the single tied probability density of all the training data. The  Mahalanobis distance of a new input from this estimated density is then used to distinguish OODs from ID samples. It attains the true negative rate (TNR) of 39.09\% at  the 95\% true positive rate (TPR). It could not detect OODs 
     in clusters B and C, as shown in Figure~\ref{fig:failure_toy_ex}(a).
     \item Softmax prediction probability (SPB)~\citep{baseline}: Figure~\ref{fig:failure_toy_ex}(b) shows that the SPB method cannot  detect the OODs in cluster A. The TNR ( at 95\% TPR) reported by the SPB technique is 60.91\%.  
     \item Class-wise Principal Component Analysis (PCA)~\citep{pca}: We performed PCA of the two classes separately in the penultimate feature space and used the minimum reconstruction error to detect OODs. 
     %The minimum reconstruction error from the principal component of the two classes was used to distinguish OODs from the ID samples. 
     This obtained  TNR of 80.91\% (at 95\% TPR). But it could not detect the OODs in cluster C, as illustrated in Figure~\ref{fig:failure_toy_ex}(c). 
     \item K-Nearest Neighbor (kNN)~\citep{dknn}:  We also used non-conformance (measured as entropy of features in the penultimate layer) in the labels of the nearest neighbors from the ID samples to detect OODs. 
     The TNR (at 95\% TPR) reported by this technique was 15\%. As shown in Figure~\ref{fig:failure_toy_ex}(d), this technique cannot  detect OODs in clusters A and B. 
\end{itemize} 












\noop{
\section{OOD Taxonomy and Existing Detection Methods}

Beyond the simple characterization of OOD samples as anomalous inputs with respect to the training data, we adopt the top-down inference for a more fine-grained definition of OOD that takes into account the prediction of the DNN model on the input in determining whether it is OOD or not. This ensures we can take into account both the epistemic and aleatoric uncertainty~\citep{uncertainty}, and enables the use of distributions learned individually over the training samples of each class along with the tied distribution learned across classes.
\label{sec:taxonomy}
\subsection{Taxonomy of OODs}
%Uncertainty in the prediction of a classifier can be used to detect OODs. We consider aleatory and epistemic as the two sources of this uncertaint. 
% Epistemic uncertainty arises due to the lack of the classifier's knowledge (such as limited training data) whereas aleatory uncertainty is due to the stochasticity (or randomness) involved in its prediction.  
DNN models predict the class of a new input based on the learned classification boundaries between the distribution of training samples of different classes. Aleatory uncertainty occurs in the regions where these distributions overlap for multiple classes, and epistemic uncertainty occurs in the regions where the probability of a sample belonging to any of the class distributions is low~\citep{ML-uncertainty-survey}. 
The uncertainty in the classifier's prediction can thus be quantified with a distance measure from the distribution(s) of the training samples. A sample lying close to multiple classes forms the source of aleatory uncertainty and a sample lying far from all the class distributions forms the source of epistemic uncertainty. In the latter case, the distribution of the training samples can be approximated either by a single tied distribution of the entire dataset or class-wise distributions defined by different classes in the dataset. 

Let there be $k$ classes $c_1, c_2, \ldots, c_k$ and the distribution of training data for each class is $p(x | c_i)$. The overall training distribution is denoted by $p(x)$. Now, given a new input $\newinp$ to the trained DNN model $M$, let $\newclass = M(\newinp)$ denote the predicted class. If $\newinp$ is an OOD, we can identify it using the following three criteria. Figure~\ref{fig:OOD_types} demonstrates different types of OOD which differ along these criteria. 
\begin{enumerate}[noitemsep,topsep=0pt,leftmargin=*]
    \item Is the OOD input having higher epistemic or aleatoric uncertainty, that is, is the input away from all training data or is it unusually more confusing? 
    \item Is the epistemic uncertainty of the OOD input unconditional or it it conditioned on the class predicted by the DNN model?
    \item Is the OOD an outlier due to unusually high deviation in the principal components of the data or due to small deviation in the non-principal (and hence, invariant) components? 
\end{enumerate}


\begin{figure}[!h]
\centering
\includegraphics[scale=.45]{figures/OOD-flow.png}
\caption{OODs with High Epistemic and Aleatoric Uncertainty}
\label{fig:OOD_flow}
\end{figure}




\noop{
Table~\ref{table:OOD_types} summarizes the taxonomy of OODs based on the distance from the ID and the source of uncertainty. In case of a single tied ID, the only source of uncertainty is the epistemic uncertainty. We classify those samples that lie far from the approximated tied ID as the OODs due to the epistemic uncertainty in the tied ID. Examples of these types of OODs are shown as the black colored OODs in Figure~\ref{fig:OOD_types}. In case of class-wise distribution of the training samples, both epistemic and aleatory can be the source of uncertainty. We classify the samples lying close to multiple class distributions as the OODs due to the aleatory uncertainty in the class-wise ID. Examples of these OODs are shown as the red colored OODs in Figure~\ref{fig:OOD_types}. Those samples that lie far from all the class distributions are classified as the OODs due to the epistemic uncertainty in the class-wise distribution of the ID. Examples of these OODs are shown as the brown, magenta and orange colored OODs in Figure~\ref{fig:OOD_types}. 

\begin{table}[!h]
\caption{Taxonomy of OODs}
\label{sample-table}
\begin{center}
\begin{tabular}{lll}
\multicolumn{1}{c}{\bf OOD Type}  &\multicolumn{1}{c}{\bf Source of uncertainty}
\\ \hline \\
Far from tied ID                                   & Epistemic\\
Far from all classes in class-wise ID              & Epistemic\\
Close to multiple class in class-wise ID           & Aleatory\\

\end{tabular}
\end{center}
\label{table:OOD_types}
\end{table}
}

%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################


%\subsection{Decomposed Distribution of OODs}

While measuring the distance of a new sample from the learned distribution to estimate $p(\newinp|\newclass)$, we can decompose the input and the training data into a set of orthogonal components and then weigh the component-wise distance from the learned distributions based on the variance of training data along different components. Outliers can have small variance around invariant components or unusually large variance around principle components.
%Decomposing the data along different components with different levels of variation in the training data enables decomposed specification of outliers, and 
%Directly computing outlier metrics such as Mahalanobis distance in the original dimensions of the input does not distinguish between .





%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################
%##########################################################################


\subsection{Limitation of Existing OOD Detection Approaches}
Different approaches differ in their ability to detect a different class of OODs described in the previous section. First, OOD detection techniques based on density estimation of the tied ID model all of the training data without considering the class of datapoints. Hence, these cannot detect OODs due to the aleatory or epistemic uncertainty in the class-wise distribution.
The tied distribution over-approximates the ID data to learn a single distribution and cannot recognize inputs as being confusing between different classes. Second, OOD detection techniques based on the softmax scores can detect OODs with high aleatoric uncertainty and inter-class confusion. But these are unable to detect the OODs with epistemic uncertainty in the tied ID. This is because of the high softmax scores usually assigned to the samples lying far from the classification boundary by the DNN classifiers. 
Third, OOD detection techniques based on density estimation of the class-wise ID might not be able to detect OODs with high aleatory uncertainty unless we perform counterfactual analysis with classes alternative to the predicted class. 
%OOD detection techniques for class-wise ID 
Finally, the techniques based on the non-conformance amongst the properties of the nearest neighbors from the training samples might not be able to detect OODs due to epistemic uncertainty (in class-wise or tied ID) whose nearest neighbors belong to the same class~\citep{dknn}.
%This is because training samples from the same class are expected to be conformant in their properties. 
\sj{Ramneet, please add references}.

\textbf{Toy dataset to analyze existing methods.} We empirically demonstrate  these limitations of existing OOD detection methods with the help of a simple 2-dimensional (2D) ID dataset with two classes. Two half-moons represent the distribution of the two classes in this dataset. We trained a classifier with three fully connected layers having 50, 2 and 2 ReLU units, respectively.
%Three blobs of data-points representing the three types of OODs were used in this example. 
Figure~\ref{fig:toy_ex} shows the dataset and the three blobs of OODs in the 2D input and the 2D penultimate feature space of the classifier. The black, brown and red colored blobs of OODs shown in the input space  represent the OODs due to epistemic uncertainty in the tied ID, epistemic uncertainty in the class-wise ID and aleatory uncertainty in the class-wise ID, respectively. The figure also shows the classifier boundary with the softmax scores in the input space.

\begin{figure}[!h]
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/section-3/input_with_OOD_types.pdf}
  \caption{}
  %\label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{0.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/section-3/penul_input_with_OOD_types.pdf}
  \caption{}
  %\label{fig:sfig1}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/section-3/classifier_boundary.pdf}
  \caption{}
  %\label{fig:sfig2}
\end{subfigure}
\caption{We use two half-moons to represent the distribution of the two classes in a 2D  dataset. (a) shows the ID samples and the three blobs of OODs in the 2D input space. (b) shows the ID samples and the OODs in the 2D penultimate feature space of the classier and
(c) shows the classifier boundary with softmax scores in the input space. \sj{Please remove whitespaces around pdf or in someway increase font of the text in figures.}}
\label{fig:toy_ex}
\end{figure}

We used Mahalanobis distance from the mean and covariance of the entire dataset as the OOD detection technique based on the density estimation of the tied ID. This mean and covariance was calculated from the penultimate features of the dataset rendered by the classifier. This mahalanobis distance calculated from the tied mean and tied covariance of the dataset was then used to distinguish OODs from ID samples. With the 95\% true positive rate (TPR), the true negative rate (TNR) reported by this technique was 39.09\%. As shown in Figure~\ref{fig:failure_toy_ex}(a), this OOD detection technique based on the density estimation of the tied ID could not detect OODs due to the epistemic and aleatory uncertainty in the class-wise ID.  Figure~\ref{fig:failure_toy_ex}(b) shows that the softmax score used to distinguish OODs from ID samples, again with the 95\% TPR, could not detect the OODs due to the epistemic uncertainty of the tied ID. The TNR reported by this OOD detection technique based on the classifier's softmax scores was 60.91\%.  We performed Principal Component Analysis (PCA) of the two classes separately in the penultimate feature space. The minimum reconstruction error from the principal component of the two classes was used to distinguish OODs from the ID samples.  Although a high TNR of 80.91\% at 95\% TPR was reported by this technique, it could not detect the OODs due to the aleatory uncertainty in the class-wise ID. Figure~\ref{fig:failure_toy_ex}(c) shows the failure of this OOD detection technique based on the density estimation of the individual classes in the dataset. We also used non-conformance in the labels of the nearest neighbors from the ID samples to detect OODs. The entropy of this label distribution in the penultimate feature space was used as a distinguishing measure between the ID samples and OODs. With 95\% TPR, the TNR reported by this technique was 15\%. As shown in Figure~\ref{fig:failure_toy_ex}(d), this technique could not detect OODs due to epistemic uncertainty in both tied and class-wise ID. 

\begin{figure}[t]
  \centering
  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the density estimation technique of tied ID to detect OODs due to epistemic and aleatory uncertainty in the class-wise distribution.}
      {\includegraphics[width=1\linewidth]{figures/section-3/mahala_tied_dist_penul.pdf}}
  \end{minipage}\quad
  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the softmax score based technique to detect OODs due to epistemic uncertainty in tied ID}
      {\includegraphics[width=1\linewidth]{figures/section-3/base_classifier_boundary.pdf}}

  \end{minipage}

\bigskip

  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the density estimation technique of the class-wise ID to detect OODs due to aleatory uncertainty in class-wise ID}
      {\includegraphics[width=1\linewidth]{figures/section-3/pca_penul.pdf}}

  \end{minipage}\quad
  \begin{minipage}{.48\linewidth}
    \centering
    \subcaptionbox{Failure of the technique based on the non-conformance among the labels of the nearest neighbors in the dataset to detect OODs due to epistemic uncertainty in both tied and class-wise in-distribution}
      {\includegraphics[width=1\linewidth]{figures/section-3/knn_label_conf_penul.pdf}}

  \end{minipage}
\caption{Different OOD detection techniques differ in their ability to detect different types of OODs. \sj{Please increase text fonts without increasing the figure size - increase font size when you are exporting to pdf - also see if you have extra whitespace around figures.}}
\label{fig:failure_toy_ex}
\end{figure}
}



==> taxonomy.tex <==
\section{Taxonomy of OODs due to Uncertainty}
\label{sec:taxonomy}
Here, we formalize the definition of OODs due to the predictive uncertainty of classifiers, namely aleatoric and epistemic uncertainty.

\textbf{OODs due to aleatoric uncertainty.} Aleatoric uncertainty of a classifier can be captured by high entropy in the prediction of the class for an input. For instance, low KL-divergence between the distribution of the predicted softmax scores for an input and the uniform distribution indicates high aleatoric uncertainty in the prediction of the classifier for that input~\citep{formal_eu_au}. For a given threshold $\delta_a$ on the entropy in the predicted probability distribution of the class, OODs due to aleatoric uncertainty are defined as follows. With $n_c$ as the number of classes, an input $x$ is an OOD due to aleatoric uncertainty if: 

\begin{equation}
    -\sum_{i=1}^{n_c} p_{i|x} \ \log\ p_{i|x} > \delta_a
\end{equation}

Note that the probability distribution 
on the prediction of the class for an input can be obtained from any layer, i.e. $p_{i|x}| 1\leq i \leq n$ is not restricted to the Softmax layer of the classifier. For instance, class labels of the nearest neighbors in the feature space (from any layer) of the classifier can also be used to predict the probability distribution of the class for an input~\citep{dknn}.

\textbf{OODs due to epistemic uncertainty.} An input lying in the low density region of the ID density indicates high epistemic uncertainty for that input~\citep{formal_eu_au,eu_ae,ML-uncertainty-survey}. Probability density function (PDF) $q$ representing the ID density can thus be used to detect OODs due to high epistemic uncertainty. For a given threshold $\delta_e$ on the probability of an input $x$ belonging to the ID density, $x$ is an OOD due to epistemic uncertainty if:

\begin{equation}
    q(x) < \delta_e
\label{eq_tied}
\end{equation}

One can also consider either only principal (or non-principal) components in the PDF for ID to detect OODs due to high (or small) deviation in the principal (or non-principal) components of the ID data. With $q_{p}$ (or $q_{n}$) as the PDF with only principal (or non-principal) components and $\delta_{ep}$ (or $\delta_{en}$) as the threshold on the probability of the input belonging to the ID density due to the principal (or non-principal) components, OODs due to high epistemic uncertainty can are defined as:
\begin{equation}
    q_{p}(x) < \delta_{ep} \vee q_{n}(x) < \delta_{en}\  \textrm{where} \  \delta_{ep} > \delta_{en}
\label{eq_p_np_tied}
\end{equation}

While considering only principal (or non-principal) components in the PDF of ID, the other term in the above equation corresponding to the non-principal (or principal) components is considered False. In other words, the input is assumed to be ID along those components for which it is not tested. However, if analysis is performed for both the components separately (instead of together as in Equation~\ref{eq_tied}), then the input is defined as an OOD if either of the two conditions in the above equation is true.

Note that $q(x)$ defined so far is for the tied (or single) ID. For class-conditional ID density, we will have a set $\{q_i(x)\ | \ 1 \leq i \leq n_c \}$ for PDFs for each class and OODs due to high class-conditional epistemic uncertainty can thus be defined as follows:

\begin{equation}
    \max_{i=1}^{n_c}\{q_i(x)\} < \delta_e
\label{eq_cc}
\end{equation}

Similarly, considering only principal $\{q_{pi}(x)\ | \ 1 \leq i \leq n_c \}$ (or non-principal $\{q_{ni}(x)\ | \ 1 \leq i \leq n_c \}$) components in defining the class-conditional ID density, an input $x$ is any OOD if:

\begin{equation}
    \max_{i=1}^{n_c}\{q_{pi}(x)\} < \delta_{ep} \vee \max_{i=1}^{n_c}\{q_{ni}(x)\} < \delta_{en} \ \textrm{where} \  \delta_{ep} > \delta_{en}
\label{eq_p_np_cc}
\end{equation}

Note that Equations~\ref{eq_tied} and~\ref{eq_p_np_tied} are the special case of Equations~\ref{eq_cc} and~\ref{eq_p_np_cc} respectively where the size of the sets representing the PDF of ID is equal to 1. Also, Equations~\ref{eq_tied} and~\ref{eq_cc} are a special case of Equations~\ref{eq_p_np_tied} and~\ref{eq_p_np_cc} respectively, when we do not consider dimensionality reduction, i.e. all components are considered as principal components in the PDF of ID. 



